CreativeSynth: Cross-Art-Attention for Artistic Image Synthesis with Multimodal Diffusion

Although remarkable progress has been made in image style transfer, style is just one of the components of artistic paintings. Directly transferring extracted style features to natural images often results in outputs with obvious synthetic traces. This is because key painting attributes including layout, perspective, shape, and semantics often cannot be conveyed and expressed through style transfer. Large-scale pretrained text-to-image generation models have demonstrated their capability to synthesize a vast amount of high-quality images. However, even with extensive textual descriptions, it is challenging to fully express the unique visual properties and details of paintings. Moreover, generic models often disrupt the overall artistic effect when modifying specific areas, making it more complicated to achieve a unified aesthetic in artworks. Our main novel idea is to integrate multimodal semantic information as a synthesis guide into artworks, rather than transferring style to the real world. We also aim to reduce the disruption to the harmony of artworks while simplifying the guidance conditions. Specifically, we propose an innovative multi-task unified framework called CreativeSynth, based on the diffusion model with the ability to coordinate multimodal inputs. CreativeSynth combines multimodal features with customized attention mechanisms to seamlessly integrate real-world semantic content into the art domain through Cross-Art-Attention for aesthetic maintenance and semantic fusion. We demonstrate the results of our method across a wide range of different art categories, proving that CreativeSynth bridges the gap between generative models and artistic expression. Code and results are available at https://github.com/haha-lisa/CreativeSynth.

==> Figures/ablation_wo.tex <==
\begin{figure}%[btp]
    \centering
    \includegraphics[width=\linewidth]{Images/ablation1}
    \caption{Results of ablation study on (a) AdaIN, inversion, and IPA, (b) IPA scale, and (c) guidance scale.}
    \label{fig:ablation_wo}    \label{fig:ablation_ip_adapter_scale}
    \label{fig:ablation_guidance_scale}
\end{figure}


==> Figures/overview.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.9\linewidth]{Images/overview.png}
 % \vspace{-15pt}
\caption{CreativeSynth overview. Different modalities naturally emerge in response to the same data source, and CreativeSynth connects all of these modalities into a common embedding space, enabling new emergent alignments and functionality.
}
\label{fig:overview}
\end{figure*}

